Non-clairvoyant Scheduling of Coflows

The coflow scheduling problem is considered: given an input/output switch with each port having a fixed capacity, find a scheduling algorithm that minimizes the weighted sum of the coflow completion times respecting the port capacities, where each flow of a coflow has a demand per input/output port, and coflow completion time is the finishing time of the last flow of the coflow. The objective of this paper is to present theoretical guarantees on approximating the sum of coflow completion time in the non-clairvoyant setting, where on a coflow arrival, only the number of flows, and their input-output port is revealed, while the critical demand volumes for each flow on the respective input-output port is unknown. The main result of this paper is to show that the proposed BlindFlow algorithm is $8p$-approximate, where $p$ is the largest number of input-output port pairs that a coflow uses. This result holds even in the online case, where coflows arrive over time and the scheduler has to use only causal information. Simulations reveal that the experimental performance of BlindFlow is far better than the theoretical guarantee.

==> Introduction_old.tex <==
\section{Introduction}

Co-flow scheduling is a recent popular networking
abstraction introduced to capture application-level computation and communication
patterns in data centers. For example, in distributed/parallel processing systems such as MapReduce \cite{dean2008mapreduce} or Hadoop \cite{shvachko2010hadoop}, Dryad \cite{isard2007dryad}, jobs/flows alternate between computation and communication stages, where a new stage cannot start until all the required sub-jobs/flows have been processed in the preceding stage. 
Therefore, the metric of performance is the delay seen by the last finishing job/flow in a stage unlike the conventional latency notion of per-job/flow delay. 

To better abstract this idea, a {\it co-flow} \cite{coflow} is defined that consists of a group of flows, where the group is identified by the computation requirements. The completion time of a co-flow is defined to be the completion time of the flow that finishes last in the group. The main ingredients of the basic scheduling problem are as follows. There is a switch with $m$ input and $n$ output ports, and each port can process jobs at a certain maximum capacity. Co-flows arrive over time, where each co-flow has a certain weight (measures relative importance) and each flow of a co-flow corresponds to a certain demand volume that has to be processed over a particular input-output port pair. 
Among the currently outstanding co-flows, the schedulers' job is to assign processing rates for all flows (on respective input-output ports), subject to ports' capacity constraints, with the objective of minimizing the weighted sum of the co-flow completion time.


The co-flow scheduling problem (CSP) is NP-hard, since a special case of this problem,  the concurrent open shop (COS) problem is NP-hard. With the COS problem, there is a set of parallel servers, and each arriving job needs to get a required amount of service from each server, and the objective is to minimize the sum of the job completion time, where the completion time of a job is defined to be the time at which it has received required service from all servers it needs. Thus, the best hope of solving the CSP is to find tight approximations. 
For the COS problem, the best known approximation ratio is $2$ that is also known to be tight. 

Work in approximating the CSP
began with intuitive heuristic algorithms such as Varys \cite{varys}, Baraat \cite{baraat}, and Orchestra \cite{orchestra} that showed reasonable empirical performance, which was then followed by theoretical work that showed that a $5$-approximation is possible \cite{shafiee}, however, no tight lower bounds better than $2$ are known yet. In further work \cite{sincronia}, a $12$ approximation was derived which also holds for the online case, when co-flows arrive over time.

In most of the prior work, a clairvoyant setting was considered, which means that as soon as a co-flow arrives, the demand volumes for each of its flows per input-output port are also revealed, which can be used to find the schedule. In general, this may not always be possible as argued in \cite{aalo} for various cases, such as pipelining used between different stages of computation \cite{isard2007dryad, condie2010mapreduce, rossbach2013dandelion} or task failures/speculation \cite{zaharia2012resilient, isard2007dryad, dean2008mapreduce}. Moreover, not assuming the exact demand volume makes the problem more robust.  


Thus, in this paper, we consider a more general setting, called {\it non-clairvoyant}, where on a co-flow arrival, only the number of flows, and their corresponding input-output port is revealed, while the 'critical parameter' the demand volumes for each flow on the respective input-output port is unknown. Any flow departs from the system as soon as its demand volume is satisfied. The departure is then notified to the algorithm.

Non-clairvoyant model for CSP has been considered in \cite{aalo}, where a heuristic algorithm {\it Aalo} has been proposed that shows reasonable empirical performance. The objective of this paper is to present theoretical guarantees on approximating the non-clairvoyant CSP. 
Their is significant work on non-clairvoyant scheduling in the theoretical computer science literature, for example for makespan minimization \cite{brecht1997competitive, he2008provably}, average stretch \cite{becchetti2000scheduling}, flowtime \cite{kalyanasundaram2003minimizing, becchetti2004nonclairvoyant}, flowtime plus energy minimization with speed scaling \cite{gupta2010nonclairvoyantly, gupta2012scheduling}, or with precedence constraints \cite{ngarg}, but to the best of our knowledge not on the CSP. 


For the non-clairvoyant CSP, we propose an algorithm that we call BlindFlow, that allocates rates to each non-departed flow in the following manner:  let the set of flows be $\mathsf{F}_{i,j}$ (across different co-flows) that need to use the same input-output port pair $(i,j)$ and weight of flow $f\in \mathsf{F}_{i,j}$ be the weight of the co-flow that $f$ belongs to. Then the rate allocated to flow $f$ is equal to the ratio of the weight $f$ and the sum of the weights of all other flows of $\mathsf{F}$. BlindFlow is clearly non-clairvoyant, online (does not need to know the future co-flow arrival infomation) and is very easy to implement. 

The other non-clairvoyant algorithm Aalo proposed in \cite{aalo} instead maintains priority queues, and a newly arrived co-flows are assigned highest priority. If demands were known, typically, flows with shorter demands are scheduled first.
Aalo tries to estimate the demand sizes by their processing time, and priority of a co-flow is decreased once the amount of time for which it has been processed and yet not finished crosses a threshold. Co-flows with identical priority are treated equally using a FIFO discipline.

Let $p_c$ be the number of distinct input-output port pairs that all flows in a co-flow $c$ need to use, and let $p=\max_c p_c$. Thus, $p$ is the largest number of ports any co-flow uses.
The {\bf main result} of this paper is to show that the BlindFlow algorithm is $8p$ approximate. This result holds even in the online case, i.e., when co-flows arrive at arbitrary time instants, as long as the completion time is counted from absolute time $0$. Completion time if defined as the difference between the finish time and the arrival time of a co-flow is called the flow-time,  is hard to even approximate even for the clairvoyant setting. As a corollary of our result, we get that the BlindFlow algorithm is $4p$ approximate for the special case of the COS problem in the non-clairvoyant setting, which to the best of our knowledge was not known.  

The derived approximation guarantee for the BlindFlow algorithm is in fact with respect to a clairvoyant {\it fractional} optimal algorithm and not just the best non-clairvoyant algorithm. 
The proof technique to derive our result involves expressing the clairvoyant {\it fractional} CSP  as a linear program (LP) and considering its dual. Then via primal-dual method, we couple the rates allocated by the BlindFlow algorithm to the dual variables of the clairvoyant fractional LP and then invoke weak duality, which is rather a novel idea in the CSP literature, inspired by \cite{ngarg}. 


The approximation guarantees derived in this paper depend on the problem instance via the $p$, the maximum number of port pairs a co-flow can use, and are not constant unlike the clairvoyant case. The proof ideas are, however, novel, and the bounds are theoretically useful when the maximum number of ports each co-flows uses $p$ is small or the number of total port pairs is small. Moreover, as the simulations show (both synthetic and real-world trace data based), the performance of the BlindFlow is far superior than the $8p$ approximation guarantee.




==> input.tex <==
%\usepackage{fancyhdr}
%\pagestyle{fancy}
%
%\usepackage{amsfonts}
%\usepackage{times}
%\usepackage[pdftex]{graphicx}
%\usepackage{mathtools}
%%\usepackage[dvips]{graphics}
%\usepackage{algorithm}
%\usepackage{algpseudocode}
%
%\usepackage{tikz}
%\usepackage{pgfplots}
%\usetikzlibrary {positioning}
%\usetikzlibrary{shapes,snakes}
%\usetikzlibrary{arrows,calc}
%\usepackage{relsize}
%\usetikzlibrary{patterns}
%\usepackage{enumitem}
%
%%\usepackage[margin=15mm]{geometry}
%
%\usepackage{arrayjobx}
%\usepackage{trimspaces}
%
%    \makeatletter
%    \def\trimspace#1{\trim@spaces@in{#1}}
%    \makeatother
%\usepackage{tcolorbox}
%
%\usepackage{longtable}
%\usepackage{lipsum}
%%\DeclareGraphicsExtensions{.jpg}
%%\usepackage[dvips]{graphicx}
%%\DeclareGraphicsExtensions{.eps}
%%\usepackage{dsfont}
%%\usepackage[T1]{fontenc}
%%\usepackage[utf8]{inputenc}
%%\usepackage{babel}
%\usepackage{appendix}
%%\usepackage{blindtext}
%
%\usepackage{amssymb}
%\usepackage{amsmath}
%\usepackage{cite}
%\usepackage{verbatim}
%\usepackage{braket}
%\usepackage{subfigure}
%\newtheorem{thm}{Theorem}[section]
%\newtheorem{definition}{Definition}[section]
%\usepackage{epsfig}
% \usepackage{epstopdf}
% \usepackage{psfrag}
% \usepackage{color}
%\epstopdfsetup{outdir=./}
%\graphicspath{{../}}
% 
% \usepackage{subfigure}
%%\usepackage{eps}
%\usepackage{amsmath,amssymb}
%%\usepackage{graphicx}
%\usepackage{color}
%\usepackage{cite}
%\usepackage{multirow,tabularx}
%\usepackage{ifthen}
%% Add these after the document class declaration
%\usepackage{times}
%%\usepackage{graphicx}
%\usepackage{amsbsy} 
%\usepackage{epsfig}
%\usepackage{color}
%\usepackage{epstoeps}
%
%\DeclareGraphicsRule{.pstex}{eps}{*}{}
% \DeclareGraphicsRule{.epstex}{pdf}{*}{}
%
%\usepackage{stackrel}
%
%
%\usepackage{amsfonts}
%\usepackage{stfloats}
%
%\usepackage[all]{xy}

 
%\DeclareGraphicsRule{.pstex}{eps}{*}{}
 %\DeclareGraphicsRule{.epstex}{pdf}{*}{}

%\usepackage{makeidx} %originally not
%\makeindex %originally not

\newcommand{\marceau}[1]{\color{black}#1\color{black}}


%\newtheorem{acknowledgement}[thm]{Acknowledgement}
%\newtheorem{algorithm}[thm]{Algorithm}
\newtheorem{assumption}[thm]{Assumption}
\newtheorem{axiom}[thm]{Axiom}
\newtheorem{case}[thm]{Case}
\newtheorem{claim}[thm]{Claim}
\newtheorem{conclusion}[thm]{Conclusion}
\newtheorem{condition}[thm]{Condition}
\newtheorem{conjecture}[thm]{Conjecture}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{criterion}[thm]{Criterion}
\newtheorem{defn}[thm]{Definition}
\newtheorem{example}[definition]{Example}
\newtheorem{exercise}[thm]{Exercise}
\newtheorem{fact}[thm]{Fact}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{notation}[thm]{Notation}
\newtheorem{problem}[thm]{Problem}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{solution}[thm]{Solution}
\newtheorem{summary}[thm]{Summary}
\newtheorem{remark}[thm]{Remark}
\newtheorem{rem}[thm]{Remark}

\newcommand{\Example}[1]{
{
\begin{tcolorbox}
\begin{quote}
#1
\end{quote}
\end{tcolorbox}
}}


\newenvironment{proof}{ \textbf{Proof:} }{ \hfill $\Box$}

\newcommand{\figref}[1]{{Fig.}~\ref{#1}}
\newcommand{\tabref}[1]{{Table}~\ref{#1}}
\newcommand{\bookemph}[1]{ {\em #1}}
\newcommand{\Ns}{N_s}
\newcommand{\Ut}{U_t}
\newcommand{\fig}[1]{Fig.\ \ref{#1}}
\def\onehalf{\frac{1}{2}}
\def\etal{et.\/ al.\/}
\newcommand{\bydef}{\triangleq}
\newcommand{\tr}{tr}


% blackboard lowercase
\def\bydef{:=}
\def\bba{{\mathbb{a}}}
\def\bbb{{\mathbb{b}}}
\def\bbc{{\mathbb{c}}}
\def\bbd{{\mathbb{d}}}
\def\bbee{{\mathbb{e}}}
\def\bbff{{\mathbb{f}}}
\def\bbg{{\mathbb{g}}}
\def\bbh{{\mathbb{h}}}
\def\bbi{{\mathbb{i}}}
\def\bbj{{\mathbb{j}}}
\def\bbk{{\mathbb{k}}}
\def\bbl{{\mathbb{l}}}
\def\bbm{{\mathbb{m}}}
\def\bbn{{\mathbb{n}}}
\def\bbo{{\mathbb{o}}}
\def\bbp{{\mathbb{p}}}
\def\bbq{{\mathbb{q}}}
\def\bbr{{\mathbb{r}}}
\def\bbs{{\mathbb{s}}}
\def\bbt{{\mathbb{t}}}
\def\bbu{{\mathbb{u}}}
\def\bbv{{\mathbb{v}}}
\def\bbw{{\mathbb{w}}}
\def\bbx{{\mathbb{x}}}
\def\bby{{\mathbb{y}}}
\def\bbz{{\mathbb{z}}}
\def\bb0{{\mathbb{0}}}
\def\b1{{\mathbf{1}}}


% Bold lowercase
\def\bydef{:=}
\def\ba{{\mathbf{a}}}
\def\bb{{\mathbf{b}}}
\def\bc{{\mathbf{c}}}
\def\bd{{\mathbf{d}}}
\def\bee{{\mathbf{e}}}
\def\bff{{\mathbf{f}}}
\def\bg{{\mathbf{g}}}
\def\bh{{\mathbf{h}}}
\def\bi{{\mathbf{i}}}
\def\bj{{\mathbf{j}}}
\def\bk{{\mathbf{k}}}
\def\bl{{\mathbf{l}}}
\def\bm{{\mathbf{m}}}
\def\bn{{\mathbf{n}}}
\def\bo{{\mathbf{o}}}
\def\bp{{\mathbf{p}}}
\def\bq{{\mathbf{q}}}
\def\br{{\mathbf{r}}}
\def\bs{{\mathbf{s}}}
\def\bt{{\mathbf{t}}}
\def\bu{{\mathbf{u}}}
\def\bv{{\mathbf{v}}}
\def\bw{{\mathbf{w}}}
\def\bx{{\mathbf{x}}}
\def\by{{\mathbf{y}}}
\def\bz{{\mathbf{z}}}
\def\b0{{\mathbf{0}}}

% Bold capital letters
\def\bA{{\mathbf{A}}}
\def\bB{{\mathbf{B}}}
\def\bC{{\mathbf{C}}}
\def\bD{{\mathbf{D}}}
\def\bE{{\mathbf{E}}}
\def\bF{{\mathbf{F}}}
\def\bG{{\mathbf{G}}}
\def\bH{{\mathbf{H}}}
\def\bI{{\mathbf{I}}}
\def\bJ{{\mathbf{J}}}
\def\bK{{\mathbf{K}}}
\def\bL{{\mathbf{L}}}
\def\bM{{\mathbf{M}}}
\def\bN{{\mathbf{N}}}
\def\bO{{\mathbf{O}}}
\def\bP{{\mathbf{P}}}
\def\bQ{{\mathbf{Q}}}
\def\bR{{\mathbf{R}}}
\def\bS{{\mathbf{S}}}
\def\bT{{\mathbf{T}}}
\def\bU{{\mathbf{U}}}
\def\bV{{\mathbf{V}}}
\def\bW{{\mathbf{W}}}
\def\bX{{\mathbf{X}}}
\def\bY{{\mathbf{Y}}}
\def\bZ{{\mathbf{Z}}}

% Blackboard capital letters
\def\bbA{{\mathbb{A}}}
\def\bbB{{\mathbb{B}}}
\def\bbC{{\mathbb{C}}}
\def\bbD{{\mathbb{D}}}
\def\bbE{{\mathbb{E}}}
\def\bbF{{\mathbb{F}}}
\def\bbG{{\mathbb{G}}}
\def\bbH{{\mathbb{H}}}
\def\bbI{{\mathbb{I}}}
\def\bbJ{{\mathbb{J}}}
\def\bbK{{\mathbb{K}}}
\def\bbL{{\mathbb{L}}}
\def\bbM{{\mathbb{M}}}
\def\bbN{{\mathbb{N}}}
\def\bbO{{\mathbb{O}}}
\def\bbP{{\mathbb{P}}}
\def\bbQ{{\mathbb{Q}}}
\def\bbR{{\mathbb{R}}}
\def\bbS{{\mathbb{S}}}
\def\bbT{{\mathbb{T}}}
\def\bbU{{\mathbb{U}}}
\def\bbV{{\mathbb{V}}}
\def\bbW{{\mathbb{W}}}
\def\bbX{{\mathbb{X}}}
\def\bbY{{\mathbb{Y}}}
\def\bbZ{{\mathbb{Z}}}

% Caligraphic capital letters
\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}


\def\cd{\mathcal{d}}

% Sans serif capital letters
\def\sfA{\mathsf{A}}
\def\sfB{\mathsf{B}}
\def\sfC{\mathsf{C}}
\def\sfD{\mathsf{D}}
\def\sfE{\mathsf{E}}
\def\sfF{\mathsf{F}}
\def\sfG{\mathsf{G}}
\def\sfH{\mathsf{H}}
\def\sfI{\mathsf{I}}
\def\sfJ{\mathsf{J}}
\def\sfK{\mathsf{K}}
\def\sfL{\mathsf{L}}
\def\sfM{\mathsf{M}}
\def\sfN{\mathsf{N}}
\def\sfO{\mathsf{O}}
\def\sfP{\mathsf{P}}
\def\sfQ{\mathsf{Q}}
\def\sfR{\mathsf{R}}
\def\sfS{\mathsf{S}}
\def\sfT{\mathsf{T}}
\def\sfU{\mathsf{U}}
\def\sfV{\mathsf{V}}
\def\sfW{\mathsf{W}}
\def\sfX{\mathsf{X}}
\def\sfY{\mathsf{Y}}
\def\sfZ{\mathsf{Z}}
\def\opt{\mathsf{OPT}}
\def\off{\mathsf{OFF}}



% sans serif lowercase
\def\bydef{:=}
\def\sfa{{\mathsf{a}}}
\def\sfb{{\mathsf{b}}}
\def\sfc{{\mathsf{c}}}
\def\sfd{{\mathsf{d}}}
\def\sfee{{\mathsf{e}}}
\def\sfff{{\mathsf{f}}}
\def\sfg{{\mathsf{g}}}
\def\sfh{{\mathsf{h}}}
\def\sfi{{\mathsf{i}}}
\def\sfj{{\mathsf{j}}}
\def\sfk{{\mathsf{k}}}
\def\sfl{{\mathsf{l}}}
\def\sfm{{\mathsf{m}}}
\def\sfn{{\mathsf{n}}}
\def\sfo{{\mathsf{o}}}
\def\sfp{{\mathsf{p}}}
\def\sfq{{\mathsf{q}}}
\def\sfr{{\mathsf{r}}}
\def\sfs{{\mathsf{s}}}
\def\sft{{\mathsf{t}}}
\def\sfu{{\mathsf{u}}}
\def\sfv{{\mathsf{v}}}
\def\sfw{{\mathsf{w}}}
\def\sfx{{\mathsf{x}}}
\def\sfy{{\mathsf{y}}}
\def\sfz{{\mathsf{z}}}
\def\sf0{{\mathsf{0}}}

\def\1{{\bf 1}}
\def\N{{N}}
\def\Nt{{N_t}}
\def\Nr{{N_r}}
\def\Ne{{N_e}}
\def\Ns{{N_s}}
\def\Es{{E_s}}
\def\No{{N_o}}
\def\sinc{\mathrm{sinc}}
\def\dmin{d^2_{\mathrm{min}}}
\def\vec{\mathrm{vec}~}
\def\kron{\otimes}
\def\Pe{{P_e}}
\def\SINR{{\mathsf{SINR}}}
\def\SIR{{\mathsf{SIR}}}
\def\SNR{{\mathsf{SNR}}}
\def\MI{{\mathsf{MI}}}



% Added by Takao
\def\nn{\nonumber}

% Chapter Numbers
\def\IntroChapter{Chapter 1}
\def\TCChapter{Chapter 2}
\def\MIMOChapter{Chapter 3}
\def\TWChapter{Chapter 4}
\def\CellularChapter{Chapter 5}
\def\MultiHopChapter{Chapter 6}
\def\PercolationChapter{Chapter 7}
\def\PWChapter{Chapter 8}
\def\TrCChapter{Chapter 9}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Robert's Notation Commands - Just temporary
\newcommand{\signb}{s} % not bold
\newcommand{\sig}{\mathbf{s}}
\newcommand{\Sig}{\mathbf{S}}
\newcommand{\noise}{\mathbf{v}}
\newcommand{\noisenb}{v}
\newcommand{\data}{\mathbf{y}}
\newcommand{\datanb}{{y}}
\newcommand{\Ff}{\mathsf{F}}
\newcommand{\ff}{\mathsf{f}}
\newcommand{\Hf}{\mathsf{H}}
\newcommand{\Gf}{\mathsf{G}}
\newcommand{\Ht}{\mathbf{H}}
\newcommand{\htime}{h}
\newcommand{\hfreq}{H}
\newcommand{\ftime}{f}
\newcommand{\ffreq}{F}
\newcommand{\Mt}{M_t}
\newcommand{\Mr}{M_r}
\newcommand{\evec}{\mathbf{e}}
\newcommand{\chanvec}{\mathbf{h}}
\newcommand{\symvecset}{\mathcal{S}}

%%%% Antonio's add %%%%%%%%%%%%%%%%%%%
\newcommand{\bLam}{\mathbf{\Lambda}}
\newcommand{\defeq}{\bydef}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\headrulewidth}{0.5pt}
\renewcommand{\footrulewidth}{0pt}
\newcommand{\helv}{%
    \fontfamily{phv}\fontseries{b}\fontsize{9}{11}\selectfont}
\fancyhf{}
\fancyhead[LE,RO]{\helv  \thepage}
\newenvironment{dedication}
{
   \cleardoublepage
   \thispagestyle{empty}
   \vspace*{\stretch{1}}
   \hfill\begin{minipage}[t]{0.66\textwidth}
   \raggedright
}%
{
   \end{minipage}
   \vspace*{\stretch{3}}
   \clearpage
}


% Following should be included in each chapter's base.tex with
% appropriate chapter title.

%\fancyhead[RE]{\helv  \bfseries Advanced MIMO Communication}
%\fancyhead[LO]{\helv  \bfseries CHAPTER X. Spatial Multiplexing}

